Learning Deep Time-index Models for Time Series Forecasting

Deep learning has been actively applied to time series forecasting, leading to a deluge of new methods, belonging to the class of historical-value models. Yet, despite the attractive properties of time-index models, such as being able to model the continuous nature of underlying time series dynamics, little attention has been given to them. Indeed, while naive deep time-index models are far more expressive than the manually predefined function representations of classical time-index models, they are inadequate for forecasting, being unable to generalize to unseen time steps due to the lack of inductive bias. In this paper, we propose DeepTime, a meta-optimization framework to learn deep time-index models which overcome these limitations, yielding an efficient and accurate forecasting model. Extensive experiments on real world datasets in the long sequence time-series forecasting setting demonstrate that our approach achieves competitive results with state-of-the-art methods, and is highly efficient. Code is available at https://github.com/salesforce/DeepTime.

==> tables/model-comparison.tex <==
\begin{table}[H]
\vspace{-0.1in}
  \centering
  \caption{Time-index models are defined to be models whose predictions, \(\hat{\vy}_t\), are \textit{purely} functions of the \textit{current} time-index features, \(\vtau_t\), e.g. relative time-index (1, 2, 3, ...), datetime features (minute-of-hour, week-of-day, etc.).
Historical-value models, whose predictions of future time step(s), \(\hat{\vy}_{t+1}\), are explicit functions of past observations, \((\vy_{t}, \vy_{t-1}, \ldots)\), and optionally covariates, \((\vz_{t+1}, \vz_t, \vz_{t-1}, \ldots)\), which can include exogenous time-series or even datetime features.}
% \begin{minipage}[t]{.5\linewidth}
% \center{\textbf{Time-index Models}}
% \vspace{-0.05in}
% \begin{equation*}
%   \hat{\vy}_t = f(\vtau_t)
% \end{equation*}
% \vskip -0.05in
% \textbf{E.g.}: {\shortname}, Prophet, Gaussian process
% \end{minipage}%
% \begin{minipage}[t]{.5\linewidth}
% \center{\textbf{Historical-value Models}}
% \vspace{-0.05in}
% \begin{equation*}
%     \hat{\vy}_{t+1} = f(\vy_t, \vy_{t-1}, \ldots, \vz_{t+1}, \vz_{t}, \ldots)
% \end{equation*}
% \vskip -0.05in
% \textbf{E.g.}: N-HiTS, Autoformer, DeepAR
% \end{minipage}%
    \begin{tabular}{cc}
    \toprule
    \textbf{Time-index Models} & \textbf{Historical-value Models} \\
    \midrule
    \vspace*{0.5em}
    \(\hat{\vy}_t = f(\vtau_t)\) & \(\hat{\vy}_{t+1} = f(\vy_t, \vy_{t-1}, \ldots, \vz_{t+1}, \vz_{t}, \ldots)\) \\
    \textbf{E.g.}: {\shortname}, Prophet, Gaussian process & \textbf{E.g.}: N-HiTS, Autoformer, DeepAR \\
    \bottomrule
    \end{tabular}%
    
    \label{tab:model-comparison}
\end{table}
